Blockwise Post-processing in Satellite-based Quantum Key Distribution

Free-space satellite communication has significantly lower photon loss than terrestrial communication via optical fibers. Satellite-based quantum key distribution (QKD) leverages this advantage and provides a promising direction in achieving long-distance QKD. While the technological feasibility of satellite-based QKD has been demonstrated experimentally, optimizing the key rate remains a significant challenge. In this paper, we argue that improving classical post-processing is an important direction in increasing key rate in satellite-based QKD, while it can also be easily incorporated in existing satellite systems. In particular, we explore one direction, blockwise post-processing, to address highly dynamic satellite channel conditions due to various environmental factors. This blockwise strategy divides the raw key bits into individual blocks that have similar noise characteristics, and processes them independently, in contrast to traditional non-blockwise strategy that treats all the raw key bits as a whole. Using a case study, we discuss the choice of blocks in blockwise strategy, and show that blockwise strategy can significantly outperform non-blockwise strategy. Our study demonstrates the importance of post-processing in satellite QKD systems, and presents several open problems in this direction.

==> intro.tex <==
\section{Introduction}
Quantum Key Distribution (QKD) uses the principles of quantum mechanics to enable two parties, commonly referred to as Alice and Bob, to establish a shared secret key~\cite{Pirandola20:QKD-advances}.
A fundamental characteristic of QKD is that it can detect any eavesdropping attempt, providing a level of security that is not achievable using classical cryptographic methods alone.
Despite much progress, QKD over long distance remains a challenge.
Specifically, quantum signals experience exponential loss while propagating through optical fibers, significantly restricting their travel distance. To overcome this challenge, many researchers are turning to satellite-based quantum communication,
leveraging the much lower loss in free space compared to fiber links~\cite{Chang2024:Entanglement}. While several experimental demonstrations have shown the technological feasibility of satellite-based QKD (e.g.,~\cite{wang2013direct}), much work remains in optimizing the overall QKD system performance and speed.


In general, QKD protocols operate in two distinct stages.  First is a \emph{quantum communication stage}, where users establish \emph{raw keys} using the actual quantum channel and the actual ``quantum-capable'' hardware (i.e., hardware capable of sending and measuring quantum states).  The second stage, the \emph{classical post-processing stage}, uses purely classical communication and computation to distill a secret key from the raw key data. 
The performance and efficiency of QKD can be improved in either stage. For satellite-based QKD, improvement in the second post-processing classical stage is a particularly important direction. This is because 
such changes would not require users to invest or install new quantum hardware, and hence  can be easily incorporated in existing satellite systems, even after launching the satellites. 
 

As such, we focus on the classical post-processing stage of satellite-based QKD systems in this paper. 
An interesting challenge in satellite communication
is the highly dynamic nature of the quantum channel,
caused by various environmental circumstances (e.g., time of day, weather conditions).
Such channel dynamics can significantly affect the key rate of QKD and need to be considered carefully. For example, existing studies~\cite{Erven12:turbulent,Vallone15:ARTS,Wang18:Prefixed-threshold} show that it is beneficial to discard measurements with a high quantum error rate under dynamic channel conditions, which can improve the overall key rate. 


In this paper, we present a classical post-processing approach to further improve the key rate.
In particular, we consider {\em blockwise} post-processing (referred to as key-pool segmenting in \cite{Amer24:dynamic-ICDCS}), which divides the raw key bits into multiple individual ``blocks'' based on their noise characteristics, and processes each block independently. In contrast to~\cite{Amer24:dynamic-ICDCS}, which focuses on terrestrial networks and considers only idealistic asymptotic scenarios, we use this strategy for satellite-based QKD systems in realistic {\em finite-key} scenarios.


We use a case study to investigate
the benefits of blockwise post-processing in improving key rate. In the case study, we consider a satellite-based QKD system with realistic noise and loss models, multiple satellite altitudes, and three ground station pairs.  Leveraging our finite-key results, we first identify an {\em optimal fidelity threshold} for a block of raw key bits, and show that discarding raw key bits with fidelity below this threshold leads to the best results. We then discuss the choice of blocks in a blockwise strategy, and show that a blockwise strategy leads to more secret key bits than a non-blockwise strategy.
The improvement is up to 8.6\% considering one day of data.  
Our results highlight the importance of 
designing classical post-processing techniques to improve the key rate in satellite-based QKD systems. 

The rest of the paper is organized as follows. In Section~\ref{sec:sat-QKD}, we present background on satellite-based QKD. In Section~\ref{sec:blockwise}, we describe the blockwise strategy and the key rate in finite-key scenarios. The benefits of using this post-processing strategy in satellite-based QKD are shown in Section~\ref{sec:results}. Section~\ref{sec:others} points out other promising directions for improving key rate in satellite QKD systems. Last, Section~\ref{sec:concl} concludes the paper. 



==> model.tex <==
\subsection{Quantum Channel Loss and Noise} \label{sec:model}
Dual-downlink entanglement distribution 
(see Fig.~\ref{fig:sat-QKD}) relies 
on photonic entangled-pair generation sources and free-space optical communication strategies. 
Specifically, the satellite platform contains an entanglement generation source and transmission optics to transmit entangled pairs to the two ground stations, which contain receiver optics and adaptive optics (to minimize atmospheric distortion) to receive photons from the satellite. The two ground stations must be simultaneously within the field-of-view of the satellite. The overall system (satellite and ground stations) needs to have accurate time synchronization, pointing and tracking, and classical communication links for QKD to operate successfully.       

 
Henceforth, we assume that the satellite utilizes spontaneous parametric down-conversion (SPDC) based dual-rail polarization entanglement sources that are well-studied and widely used~\cite{dhara2022heralded}.
In such entanglement sources, a two-qubit entangled Bell state requires four orthogonal modes (i.e., two pairs of modes) to encode, and takes the form  
    $\ket{\Psi^{\pm}} = \frac{1}{\sqrt{2}}(\ket{1,0;0,1}\pm\ket{0,1;1,0})$.
The vacuum state is $\ket{0,0;0,0}$. There are other spurious high-order photon states. The pump power of the source needs to be low 
so that high-order photon states are negligible.

The satellite quantum communication link  involves free-space optical (FSO) transmission, and hence the analysis of such links must account for the characteristics of the optical channel.
The transmission loss for each entangled photon scales  quadratically with free space propagation length (i.e., from the satellite to the ground) and exponentially with 
atmospheric
propagation length (i.e., from the atomospheric boundary to the ground) \cite{panigrahy2022optimal}.
FSO transmission reduces the mean photon number of the transmitted state, and can result in a pure state becoming mixed. Such effects impede the probability of successfully delivering the entangled photons to both ground stations, as well as affecting the fidelity (to the ideal entangled state) of the delivered entangled photons. Namely, it reduces the probability of receiving a perfect pair of entangled photons at the two ground stations.

In addition to transmission loss, atmospheric FSO transmission channels have to contend with a variety of noise processes. One such source of noise are the unfiltered background photons. Any excess photons in the channel will cause false events to be treated as successes, thereby impacting the fidelity of the  entangled pair that should have been delivered. The main contributor of the background photon flux is commonly associated with the brightness of the sky and varies drastically depending on the time of the day. More specifically, the level of background photon flux is at its highest during clear daylight, and at its lowest during  clear nighttime. We compute the fidelity of the generated entangled state between two ground stations by modeling the arrival of unfiltered background photons as detector dark click events.

\subsection{Improving Key Rate in Satellite-based QKD}
Real-world deployment and commercial viability of satellite-based QKD depend heavily on its key rate.
The key rate can be improved through innovative quantum technologies, 
e.g., high-performance entanglement sources, wavelength multiplexing, and high-dimensional QKD.
Another direction, which we focus on in this paper, is innovation in the classical post-processing stage, which can be designed for general quantum technologies, or customized for specific quantum hardware. 
Such post-processing innovations have the advantage that they can be easily deployed in existing systems,  even after the launch of a satellite. 

We next outline one such post-processing technique. From the above sections, it is clear that satellite QKD has several unique challenges, one of particular note being the dynamic nature of the noise in the channel due to changing environmental effects.  Recalling our discussion of the E91 protocol earlier, we see that such dynamics cause the noise level in both the $Z$ and $X$ strings (the raw keys) to vary with time.  Ordinarily, classical post-processing will treat the entire string as one homogeneous block, computing the adversary Eve's uncertainty on the entire string as a function of the average noise.  However, this gives a pessimistic key rate since, for certain, potentially large sections, of these raw keys, the noise is much lower and, thus, Eve will have potentially much less information on that particular block.  Thus, it makes sense to break the $Z$ and $X$ strings into ``blocks''---each block having an expected noise level that is homogeneous.  Error correction and privacy amplification can then be run on each block independently, assuming the blocks are of sufficient size. As we show later, this blockwise strategy can produce significant  improvement in key generation rates.



==> others.tex <==
\section{Open Problems} \label{sec:others}

Our case study in Section~\ref{sec:results} demonstrates the benefits of applying blockwise strategy 
in satellite-based QKD, and in general, the importance of carefully considering the post-processing stage to improve key rate. In the following, we discuss several open problems related to improving key rates in satellite QKD systems.  

\smallskip
\noindent{\bf Real-time dynamic channel conditions.} In addition to time-of-day effects, many other environmental factors (e.g., weather, cloud coverage) can lead to dynamic quantum channel conditions. Often times, real-time monitoring is needed to identify such dynamic conditions, estimate quantum error rates, and then divide the raw data into blocks accordingly. In addition, one needs to determine what range of error rates fall into one block so that the size of each block is sufficiently large, while the error rates of a block is not too heterogeneous.  


\smallskip
\noindent{\bf  Other components in post-processing.} 
In our blockwise strategy, after raw data are divided into blocks, error correction and privacy amplification are run for each block separately. Another approach is to bound the quantum min entropy of each block in the blockwise strategy directly, and run a single privacy amplification processes over all the blocks. That is, use a single invocation of privacy amplification, as in the non-blockwise strategy, yet still retain the benefit of increased key lengths as in blockwise post-processing. In general, the multiple components in post-processing can be jointly considered for better efficiency.


\smallskip
\noindent{\bf Connecting quantum and classical techniques.} 
While we emphasize the importance of classical post-processing  in improving key rate in satellite-based QKD, which is in parallel to quantum techniques, another direction is connecting quantum and classical techniques. For instance, for satellite systems that can tune quantum parameters (e.g., pump power, beam width), an interesting direction is to combine the choice of the parameters with the post-processing technique, and determine them jointly to optimize key rate. In addition, customized post-processing techniques can be developed for certain new quantum technologies. One example is high-dimensional QKD, which features superpositions of many (instead of two) orthogonal quantum states. This is regarded as a promising technology for satellite-based QKD since it is expected to exhibit increased channel capacity and resilience than two-dimensional systems. For such high-dimensional systems, the error characteristics of the quantum channel may differ from those for two-dimensional systems, and hence specialized post-processing techniques may benefit such systems.  


\smallskip
\noindent{\bf Other attack models.}  In Section~\ref{sec:blockwise}, we consider a standard attack model where the adversary has full control of the quantum channels from the satellite to the two ground stations. It would be interesting to consider alternative, more realistic security models (in terms of adversarial capabilities), 
and how post-processing methods can help in this context.  
For instance, it is likely Eve will not control everything and would have to launch an airborne object (e.g., a drone) to intercept incoming signals from a satellite. However, such an object would be unable to capture everything.  This was a security model introduced in \cite{ghalaii2023satellite}. How blockwise processing, or other alternative methods, can benefit key rates in this scenario is worthy of investigation.


==> perf.tex <==
\section{Benefits of Blockwise Post-processing}\label{sec:results}


\tydubfigsingle{Fidelity_alt_500_Toronto-DC.png}{$A=500$ km.}{Fidelity_alt_1300_Toronto-DC.png}{$A=1300$ km.}{Fidelity over time for Toronto-DC pair. For clarity, each point in the figure represents the average fidelity over one minute.}{fidelity}


\singlefig{secret_key_bits_vs_fidelity_threshold_Toronto_DC_nonblockwise.png}{Normalized number of secret key bits versus fidelity threshold, Toronto-DC, non-blockwise strategy.
For each altitude, the number of secret key bits is normalized by the maximum number of secret key bits (obtained using the optimal fidelity threshold) for that altitude. }{threshold}

\singlefig{Percent_of_improvement_combine_all_gs_best_value_from_2blocks_and_3blocks.png}{Improvement of  
blockwise strategy over non-blockwise strategy.
No key is generated for Toronto-Houston when the altitude is 500 km. }{improve}


We next use a case study to demonstrate the benefits of blockwise post-processing strategy. In this case study, 
we consider a polar constellation of low-earth-orbit (LEO) satellites consisting of 20
rings, each ring with 20 satellites. These satellites orbit around the Earth at the same altitude $A$, which is set to 500, 800, 1000, or 1300 km. We consider three
ground stations in North America: 
Washington D.C. (DC), Toronto, and Houston, forming a total
of three ground station pairs. 
Each satellite is equipped with an SPDC entanglement source (see Section~\ref{sec:model}) that 
generates $10^9$ entangled photons per second. 
The pump power is set to a low value of 0.01 so that high-order photon contributions are negligible.  
For  successful delivery of an entangled pair, the elevation angles between the satellite and the two ground stations need to exceed an angle, which is set to 20$^{\circ}$ in our simulation. 
When a ground station pair can be served by multiple satellites, we select the one with the highest estimated fidelity to the ground station pair.


To account for the time-of-day effects, as in \cite{Maule2024:scheduling}, we consider four time points, 12am, 6am, 12pm, and 6pm, in a day. For simplicity, we divide the entire day into four 6-hour intervals, starting respectively from the above four time points, 
and assume the same solar radiance
for each interval. The solar radiance for each of the four time points is based on the measurements for March 15, 2022~\cite{Maule2024:scheduling}.


The key rate for blockwise and non-blockwise strategies uses the finite-key results in Section~\ref{sec:blockwise}. It requires determining an optimal sampling rate, which is determined numerically.  
Specifically, for non-blockwise strategy, the sampling rate (i.e., $m/N$) is varied from $10^{-5}$ to $0.05$, 
and an optimal value is selected using grid search 
to maximize the key rate. For blockwise strategy, the optimal sampling rate for each block (i.e., $m_i/B_i$) is determined separately using grid search. 

\smallskip
\noindent{\bf Channel dynamics.} Using the quantum channel noise model, we obtain the fidelity per second (when there is at least one satellite in view of the ground station pairs).  Fig.~\ref{fig:fidelity} plots fidelity for Toronto-DC over time for two altitudes, $A=500$ km and 1300 km.
 We see that fidelity changes dynamically, roughly following four 6-hour intervals as in our assumption. 
 The first and last intervals, from 12am to 6am and from 6pm to 12am, have the highest fidelity, followed by the second interval, 6am to 12pm;  the third interval, from 12pm to 6pm, has the lowest fidelity. 
 In addition, fidelity also change within each interval due to changing satellite distance and angle from the ground stations.  


Existing studies~\cite{Erven12:turbulent,Vallone15:ARTS,Wang18:Prefixed-threshold} propose discarding measurements that have low fidelity. While it is clear that measurements with very low fidelity (e.g., significantly lower than the noise tolerance of the QKD scheme) should be discarded, it is not clear at exactly which fidelity level should the measurements be discarded for a given setting. We next investigate the choice of {\em fidelity threshold}, i.e., below which fidelity value should the raw key bits be discarded.  
Eq. (\ref{eq:keyrate-nonblock}) shows the opposing impacts of 
discarding low-fidelity raw key bits on the total number of secret key bits: on the one hand, it leads to lower error rate ($Q$); on the other hand, it leads to fewer raw key bits ($n$) and potentially higher sampling impact ($\mu$). As a result, we expect an {\em optimal fidelity threshold}: discarding raw key bits with fidelity below this threshold leads to the maximum number of secret key bits. 


Fig.~\ref{fig:threshold} plots the normalized number of secret key bits when varying the fidelity threshold from 0.70 to 0.90 for Toronto-DC, considering all the raw key bits generated in a day. The results for altitude $A=500$, 800, 1000, and 1300 km are plotted in the figure. We see that there indeed exists an optimal fidelity threshold for each setting, and the optimal values 
are similar (0.82 or 0.84) across different settings.    
Similarly, we determine the optimal fidelity thresholds for the other two ground station pairs across various altitudes.  The results presented below for each setting are obtained using the optimal fidelity threshold for that setting. In blockwise strategy, we identify optimal fidelity threshold for each block separately.

In the above, we have demonstrated the impact of fidelity threshold and identified an optimal fidelity threshold based on the fidelity of the raw key bits for each  setting. In practice, the fidelity of the raw key bits can be estimated by sampling a small number of raw bits in a short time window or using other methods (e.g.,  characterizing free-space optical links, measuring signal-to-noise ratio), which is left as future work.

\smallskip
\noindent{\bf Benefits of blockwise strategy.} We next compare the number of secret key bits under non-blockwise and blockwise strategies.
%after removing the raw bits with low fidelity. 
For blockwise strategy, we explore two methods: (i) 2-block, the first with very high fidelity ($\ge 0.98$), and the second containing the rest, and (ii) 3-block, the first with fidelity $\ge 0.98$, the second with fidelity in $(0.90,0.98)$, and the third containing the rest. From Fig.~\ref{fig:fidelity}, we see three distinct fidelity ranges, indicating that 3-block might be a good choice. On the other hand, we also need to consider the size of a block, since sampling effect is higher for smaller blocks (see Eq. (\ref{eq:mu})). Of all the settings we explore, we observe 3-block outperforms 2-block strategy in most cases. However, in some cases (e.g., Toronto-Houston, $A=800$ and 1000 km), 2-block outperforms 3-block strategy. For a given setting, finding the best blockwise strategy is an open problem that is left as future work.


Fig.~\ref{fig:improve} plots the percentage of improvement of the blockwise strategy over
the non-blockwise strategy, i.e.,  $(\ell_{\text{block}}-\ell_{\text{non-block}})/\ell_{\text{non-block}}$, where $\ell_{\text{block}}$ and $\ell_{\text{non-block}}$ denote the total number of secret key bits under blockwise (2-block or 3-block, whichever is better) and non-blockwise strategies, respectively. 
We see that blockwise strategy leads to up to $8.6\%$ 
more key bits than non-blockwise strategy. Only in one case (DC-Houston, $A=500$ km), the blockwise strategy leads to fewer keys than the non-blockwise strategy due to the small number of entanglements that are successfully received, and hence suffers from higher sampling rate; see Eq. (\ref{eq:mu}). On the other hand, when applied to 10 days of raw key bits, blockwise strategy leads to more keys than non-blockwise strategy in all settings (figure omitted), and the improvement is larger than when considering one day.    

